Evaluating the Explainability of Neural Rankers

Information retrieval models have witnessed a paradigm shift from unsupervised statistical approaches to feature-based supervised approaches to completely data-driven ones that make use of the pre-training of large language models. While the increasing complexity of the search models have been able to demonstrate improvements in effectiveness (measured in terms of relevance of top-retrieved results), a question worthy of a thorough inspection is - "how explainable are these models?", which is what this paper aims to evaluate. In particular, we propose a common evaluation platform to systematically evaluate the explainability of any ranking model (the explanation algorithm being identical for all the models that are to be evaluated). In our proposed framework, each model, in addition to returning a ranked list of documents, also requires to return a list of explanation units or rationales for each document. This meta-information from each document is then used to measure how locally consistent these rationales are as an intrinsic measure of interpretability - one that does not require manual relevance assessments. Additionally, as an extrinsic measure, we compute how relevant these rationales are by leveraging sub-document level relevance assessments. Our findings show a number of interesting observations, such as sentence-level rationales are more consistent, an increase in complexity mostly leads to less consistent explanations, and that interpretability measures offer a complementary dimension of evaluation of IR systems because consistency is not well-correlated with nDCG at top ranks.

==> figdefs/mer.tex <==
\begin{figure}
\centering
\includegraphics[width=.99\columnwidth]{figs/MRC_Passages.pdf}
\caption{Effect of number of rationales on MRC values at passage level}
\label{fig:mer}
\end{figure}


==> figdefs/mrc-document.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=.6\columnwidth]{figs/new_fidelity.pdf}
\caption{\small Effect of the number of rationales on the intrinsic explanation consistency (MRC) across different NRMs for the MS-MARCO document ranking task.}
\label{fig:doc_intrinsic}
\end{figure}


==> scratch/evalframework_old.tex <==
\section{Methodology}
Let us consider a corpus $C = \{d_1,d_2,d_3,...,d_n\}$ with n documents. For a given query $Q$ and IR model $M$ let $R = \{r_1,r_2,r_3,...,r_k\}$ be the retrieved top-$k$ ranklist. For explaining the predictions of the model, we consider a model-agnostic explainer $Exp$ that gives explaining spans of text $E_i = \{e_{i1},e_{i2},e_{i3},...,e_{il}\}$ which makes a document relevant as an output given the query $Q$, relevant document $r_i$, and IR model $M$. The set of explaining spans is calculated as $E_i = Exp(r_i, Q, M)$. To evaluate the model $M$ based on the relevance of the retrieved documents $R$, we can consider scores such as precision, recall, and mean average precision, based on the application. Let us denote this score as $S_r$. 

\subsection{Fidelity}
To evaluate the consistency of the model $M$, we calculate the relevancy score $s_{ij}$ by masking the {j}-th span $e_{ij}$ for a document $r_i$. However, a combination of text spans could have higher fidelity than individual text spans as the relevant context could be shared among the text spans. So, for a document with N spans, we consider a maximum of $m$ combination of spans such that $j \in (1, N)$. Let $s_i$ be the relevance score of the full document with respect to the query $Q$. Let $f_{ij}$  be the fidelity of span $j$. Since we also consider the combination of spans to calculate fidelity, let $c \in (C_1, C_2, ..., C_{N \choose m})$ denote the combination of spans. If $c_j$ represents the set of all combinations of spans from $c$ where j-th span is an element, then ${s_{i1},s_{i2},...,s_{ic}}$ represents the relevance scores corresponding to the pseudo documents ${d_{i1},d_{i2},...,d_{ic}}$ where each document is .
% then the difference between $s_i$ and $s_{ij}$ ($f_{ij} = |s_i-s{ij}|$) is calculated. To calculate the fidelity of each span, we mask the spans as well as the combination of spans from the document and calculate the relevance s

To calculate the consistency $C_i$ We pool the relevance scores as $C_i = mean(s_{i1},s_{i2},s_{i2},...,s_{il})$. The overall consistency of the explainable model $S_c = mean(C_1, C_2, ..., C_n)$.



\subsection{Trustworthiness}
To evaluate the trustworthiness of the model the correlation between the model-annotated scores and human-annotated scores needs to be calculated. Let $H_i = {h_{i1}, h_{i2}, h_{i3}, ...,h_{ip}}$ for a retrieved document $r_i$. We calculate the Jaccard similarity between the machine-annotated $E_i$ spans and Human annotated spans $H_i$. 

\begin{equation}
J(E_i, H_i) = \frac{(E_i\cap H_i)}{(E_i\cup H_i)}
\end{equation}

If none of the documents in the ranklist are relevant to the query, then $J(E_i, H_i) = 0$ as the human-annotated spans are not available for non-relevant documents.


==> scratch/intro.tex <==
\section{Introduction}

A paradigm shift from feature-based to data-driven end-to-end models (commonly known as deep learning \inote{cite}) has led to prolific improvements in effectiveness over a wide range of supervised learning tasks (e.g., classification \inote{cite}, regression \inote{cite}, ranking \inote{cite} etc.) involving a range of different data modalities (e.g., image \inote{cite}, text \inote{cite}, speech \inote{cite}, etc., or even their combinations \inote{cite}). However, deploying such predictive models in domains that require expert human decision making skills (e.g., a doctor diagnosing a disease \inote{cite}, or a judge deciding the verdict of a court case \inote{cite}) raises concerns related to generalisability and trustworthiness of these models. For instance, the authors of \cite{chalkidis-etal-2019-neural} show that an end-to-end attention-based hierarchical sequential modeling approach trained on examples of case descriptions (inputs) and indicators for human right violation (labels), despite performing well in terms of effectiveness, leads to high attention weights being assigned to non-pertinent segments within the documents while the pertinent sections missing the attention, e.g., a segment `police officers beat him for several hours forcing him to confess' not obtaining high attention, which in turn, shows that the model's predictive mechanism does not correlate with that of a human's thus raising concerns about the generalisability and trustworthiness of the model. 



Sometimes, providing explanations can also be required by law as mandated by regulations such as GDPR \cite{gdpr2018}, 
wherein commercially deployed AI models may now be required to `explain' to its consumers the predictive decision of a model, e.g., in cases of personalised recommendation \inote{cite}.
%Local explanations have become a popular means of generating explanations for tasks with discrete label space.

A wide range of model-agnostic local explanation approaches have been proposed for ML tasks \cite{lipton2016mythos, MontavonSM17}, most of them focusing on providing an instance-wise explanation of the output of the model as either a subset of input features \citep{anchors:aaai18, chen2018learning}, or a weighted distribution of feature importance \cite{ribeiro2016should,lundberg2017unified}. 
While the explanation space itself and methods to generate explanations are  widely known in practise for classification tasks, their utility is largely unexplored for ranking tasks.  


In recent years, neural retrieval models (NRM) have gained prominence, achieving state-of-the-art results on various document and passage ranking tasks \cite{khattab2020colbert,monot5,ance,deepct,nogueira2019doc2query}. Neural models are capable of modeling the semantic similarity between the query and document vector embeddings for the purpose of ranking, leading them to outperform traditional sparse retrieval methods, such as BM25 or language modelling based rankers, which rely on the explicit term matching between queries and documents. However, despite their success, NRMs suffer from poor \textit{interpretability} of their results~\cite{explainable-ir-survey}. With the increasing deployment of more complex NRMs, it is essential to explain the retrieval decisions of a black-box complex model to its end-users, thereby increasing their trust in the model~\cite{qu2021deep}.

Given a query, while it is straightforward to understand why a document is retrieved by a sparse retrieval model as the relevance score depends on the explicit presence of the query (or expansion) terms, the results produced by NRMs, on the other hand, are hard to interpret as these models rely on the closeness of query and document representations in the embedding space. This inherent opaqueness of NRMs make them potentially non-trustworthy to end-users, especially in critical domains such as healthcare, finance, and law~\citep{10.1145/3209978.3210193, explainable-ir-survey}. Approaches to explaining NRMs include providing additional information and explanations to the end-users such as informative snippets~\citep{explainable-elements} as well as generating terse explanations (in terms of noun phrases) describing the query aspects covered by the retrieved documents~\cite{docrelevance2search}. Alternatives include probing the feature space of the underlying models and visualizing regions in the embedding space that affect the model output~\citep{gradcam} and personalized explanations based on user characteristics~\citep{verberne2018explainable}.
Furthermore, it has been found that explanations generated by popular interpretabilty models such as LIME \cite{lime} and SHAP \cite{SHAP,deepshap} vary widely raising concern about the robustness and utility of the explanations produced by directly applying these interpretability methods to NRMs~\citep{deepshap}.





Information Retrieval helps us in retrieving the documents from corpora relevant to the given query. Many techniques have been proposed in the past few decades in this domain. However, Only a few have stood the time and are considered to be the standard baselines to date. Some of the standard baselines are BM25, ColBERT\cite{colbert}, ANCE\cite{xiong2020approximate}. BM25 uses lexical information for the purpose of retrieval whereas, neural-based techniques such as ColBERT and ANCE use semantic information. Neural-based techniques have been shown to increase the performance of the retrieval but they lack transparency as it is hard to interpret the semantic information encoded in the dense representation of the document. 

There is a need to build interpretable systems which can explain the reason behind the retrieved rank list. Especially, In the case of text retrieval, spans of text inside the documents could be an explainable factor for the retrieved documents. In this paper, we have proposed a perspective for the future research direction which focuses on evaluating the explainable information retrieval systems. The three important factors that define the performance of an explainable information retrieval system (XAIR) are as follows:
\begin{itemize}
  \item Relevancy.
  \item Consistency.
  \item Trustworthiness.
\end{itemize}
Finally, we try to give a comprehensive score that measures a XAIR system based on these factors. 


==> tables/res.tex <==
\begin{table*}[t]\centering
\caption{Results}\label{tab:summaryres}
\small
\begin{tabular}{lrrrrrrrr}\toprule
&\multicolumn{3}{c}{Passage Ranking} &\multicolumn{4}{c}{Document Ranking} \\\cmidrule{2-8}
\multirow{2}{*}{Model} &\multirow{2}{*}{Optimal parameters} &Relevance &Explainability &\multirow{2}{*}{Optimal parameters} &Relevance &Explainability &Trustworthiness \\\cmidrule{3-4}\cmidrule{6-8}
& &nDCG &MRC & &nDCG &MRC &MER \\\cmidrule{1-8}
BM25 &NA &0.491 &\textbf{0.9687} &\textbf{NA} &0.521309 &0.41228 &\textbf{0.18268} \\\cmidrule{1-8}
ColBERT &4 &0.69 &0.7621 &5 &0.567502 &0.35691 &0.16694 \\\cmidrule{1-8}
MonoT5 &6 &0.71334 &0.6650 &5 &0.60452 &0.35731 &0.17412 \\\cmidrule{1-8}
MonoElectra &6 &\textbf{0.746} &\textbf{0.7704} &5 &\textbf{0.618496} &\textbf{0.43503} &0.17451 \\\midrule
TCT-ColBERT &5 &0.69 &0.5095 &4 &0.57876 &0.3773 &0.1798 \\
\bottomrule
\end{tabular}
\end{table*}

